MuCPAD: A Multi-Domain Chinese Predicate-Argument Dataset

During the past decade, neural network models have made tremendous progress on in-domain semantic role labeling (SRL). However, performance drops dramatically under the out-of-domain setting. In order to facilitate research on cross-domain SRL, this paper presents MuCPAD, a multi-domain Chinese predicate-argument dataset, which consists of 30,897 sentences and 92,051 predicates from six different domains. MuCPAD exhibits three important features. 1) Based on a frame-free annotation methodology, we avoid writing complex frames for new predicates. 2) We explicitly annotate omitted core arguments to recover more complete semantic structure, considering that omission of content words is ubiquitous in multi-domain Chinese texts. 3) We compile 53 pages of annotation guidelines and adopt strict double annotation for improving data quality. This paper describes in detail the annotation methodology and annotation process of MuCPAD, and presents in-depth data analysis. We also give benchmark results on cross-domain SRL based on MuCPAD.

==> content/model.tex <==
\section{Model}
% 
% Besides, SRL task is generally constite of multiple subtasks: predicate identification, predicate disambiguation, argument identification and argument classification. 
% At present, predicate identification has achieved high performance. Besides, the predicates are given in word-based Chinese SRL researches popularized by CoNLL-2009. So we use given predicate which is convenient for us to compare with previous studies in the in-domain.
% In addition, our guideline needn't pre-defined frames, therefore, we just need to handle the latter two subtasks, i.e. argument identification and argument classification, which are also called argument labeling.

% Due to predicate identification has achieved high performance, and the predicates are given in word-based Chinese SRL researches popularized by CoNLL-2009 , we use the setting of given predicate.
% 给定谓词的缘由：现在的谓词识别性能很高；之前中文word based实验性能是给定谓词的，在in-domain上有助于与前人进行比较。
 

To facilitate our presentation in the following sections, we first formulate our basic SRL model. Following \cite{cai-2018A-srl}, we treat the SRL parsing task as a sequence labeling problem and introduce a "None" label to indicate that there is no semantic relationship between word and predicate.
% We build all the works over a full end-to-end model proposed by \cite{cai-2018A-srl} for word-based SRL.
As shown in Figure \ref{fig:base-model}, the model mainly contains a deep BiLSTM encoder and a biaffine attentional scorer, which is described as follows. 
\input{images/base-model}
\textbf{Input layer.}
% Due to previous studies shown that predicate-indicator can lead to superior performance (Tan et al., 2018;\cite{cai-2018A-srl}) 
 Given an input sequence $s = w_1, w_2, ..., w_n$, for each token $w_i$, we concatenate the pre-trained word embedding $\mathbf{e}_{i}^{pre}$, the randomly initialized word embedding $\mathbf{e}_{i}^{r}$, the char embedding $\mathbf{r}_{i}^{c}$ and the predicate indicator embedding $\mathbf{e}_{i}^{p}$ as our basic model input, where $\mathbf{r}_{i}^{c}$ are encoded from word characters with CNNs and $\mathbf{e}_{i}^{p}$ is used to indicate whether the word is predicate. Besides, since \citep{cai-2018A-srl} demonstrated that the impact of part-of-speech (POS) tag embedding is less compared to the previous works for this task, we remove it from the word representation. The i-th word is represented as follows:
\begin{equation} \label{eq:concate}
\mathbf{x}_i =  \mathbf{e}_{i}^{pre}\oplus \mathbf{e}_{i}^{r} \oplus    \mathbf{r}_{i}^{c} \oplus  \mathbf{e}_{i}^{p}
\end{equation} 
        
\textbf{BiLSTM encoder.} 
The model applies three-layers BiLSTM as an encoder to obtain context-aware representations of each $\mathbf{x}_{i}$, in which the output is denoted as $\mathbf{h}_{i}$. 

%The representation of the i-th word is fed into a three-layers BiLSTM to obtain context-aware representations, and we denote the output of the top-layer BiLSTM as hi. And we denote the output of the top-layer BiLSTM as $\mathbf{h}_{i}$.

\textbf{Biaffine attention role scorer.}
% Biaffine attentional scorer is used to predict all semantic role labels for all given word pairs in the sentence.
% find the highest-scoring label ($l\epsilon({L \cup None})$) of each word. 
Two separate MLPs are applied to each $\mathbf{h}_{i}$, then, we will obtain two vectors with smaller dismensionality $\mathbf{h}_{i}^{pred}$ (as predicate) and $\mathbf{h}_{i}^{arg}$ (as candidate arguments). Finally, the scores of the roles between predicate and argument is computed via a biaffine operation with two distinguish bias terms
% by following formula:
% \begin{equation} \label{eq:biaffine}
% \begin{aligned}
%  \texttt{score}(i \leftarrow j) = \mathbf{h}_{i}^\mathrm{T(arg)} 
%  \mathbf{W}^{(role)}  \mathbf{h}_{j}^{\textup (pred)}\\
%  + \mathbf{U}^{(role)}(\mathbf{h}_{i}^\mathrm{(arg)} \oplus \mathbf{h}_{j}^{\textup (pred)})\\
%  + \mathbf{b}^{(role)}
%   \end{aligned}
% \end{equation} 

\textbf{Training loss.}
For each $\mathbf{w}_{i}$ and its predicates $\mathbf{w}_{j}$ and semamtic role label $\mathbf{l}$, we minimize the negative log likelihood of the gold structure and label.
% the parser adopts local cross-entropy losses: 交叉熵和对数似然还是不一样的吧
% \begin{equation} \label{eq:biaffine}
% \begin{split}
%  \texttt{loss}(i \xleftarrow{l} j) = &-\log{
% \frac{e^{\texttt{score}(i \leftarrow j)}}
% {\sum_{0 \le k \le n} e^{\texttt{score}(i \leftarrow k)}}
% } \\ 
% & -\log{
% \frac{e^{\texttt{score}(i \xleftarrow{l} j)}}
% {\sum_{l' \in \mathcal{L}} e^{\texttt{score}(i \xleftarrow{l'} j)}}
% }
% \end{split}
% \end{equation} 

% where ${  1 \leq i \leq n}$ and ${1 \leq j \leq n}$ , 


% 在Google发布的bert-base-chinese在无标注数据和标注数据上进行多轮微调（3轮），继续使用语言模型的损失函数进行训练。无标注数据的数据分布如图所示：。

% 我们使用的是Su,首先用（）句法标注数据训练一个句法模型，然后得到
% We  employ  the  extension  of  biaffine parser proposed by Jiang et al. (2018) to train on CODT data and generate automatic dependency tree   s.



==> images/tbl-annotate-statistics.tex <==
% \setlength{\tabcolsep}{3.6pt}
% \begin{table}[tb]
% %\setlength{\leftskip}{-25pt}
% \begin{center}
% % \begin{small}
% \begin{tabular}{l  c c c c c }
% \toprule
%       &Train&Dev&Test \\
% \hline
% CoNLL & 3,796 & 5,658  & 1,784  \\[2pt]
% % \hline
% Peking & 7,521 & 11,416 & 4,107 & 7,438 & 3,750\\[2pt]
% % \hline
% total & 11,317 & 17,074 & 5,891 & 11,156 & 5624 \\[2pt]
% \hline
% % \bottomrule
% \end{tabular}
% % \end{small}
% \caption{Target data statistics in predicate number.} 
% \label{data-statistic-target}
% \end{center}
% \end{table}



\begin{table*}[tb]
\setlength{\tabcolsep}{2pt}
%\setlength{\leftskip}{-25pt}
\begin{center}
% \begin{scriptsize}
\begin{small}
% \begin{tabular}{l  l l l l l l l}
\begin{tabular}{l l l l l l l }
\toprule
% (\#Pred / \# Sent)& \multicolumn{1}{c}{Source } &{ PB }&{PC}&{ZX}&{LAW}&{MED}&{CPB2.0} \\
& News &PB &PC&ZX&LAW&MED \\
\midrule
% Train & 32,790 / 13,022 & -& - & - & - & - & 72,616 / 13,170\\[2pt]
% % \hline
% Dev & 4,098 / 1,875 & 3,796 / 1,255 & 5,658 / 1,295  & 1,784 / 492 & 3,718 / 778 & 1,874 / 478 & - \\[2pt]
% % \hline
% Test & 4,101 / 2,077& 7,521 / 2,498& 11,416 / 2,595& 4,107 / 1,083 & 7,438 / 2,035 & 3,750 / 1,414 & -\\[2pt]
% % \hline
% Total& 40,989 / 16,974 & 11,317 / 3,753 & 17,074 / 3,890& 5,891 / 1,575& 11,156 / 2,813& 5,624 / 1,892 &  72,616 / 13,170\\[0pt]

\#Sent & 40,989 & 11,317 & 17,074 & 5,891 & 11,156 & 5,624 \\
% \hline
\#Pred & 16,974 & 3,753 & 3,890 & 1,575 & 2,813 & 1,892  \\
% \hline
% Test & 4,101 / 2,077& 7,521 / 2,498& 11,416 / 2,595& 4,107 / 1,083 & 7,438 / 2,035 & 3,750 / 1,414 & \multicolumn{1}{c}{--}\\[0pt]
% \hline
% Total& 40,989 / 16,974 & 11,317 / 3,753 & 17,074 / 3,890& 5,891 / 1,575& 11,156 / 2,813& 5,624 / 1,892 &  72,616 / 13,170\\[0pt]

% Train & 32,790 (13,022) & \multicolumn{1}{c}{--} & \multicolumn{1}{c}{--} & \multicolumn{1}{c}{--} & \multicolumn{1}{c}{--} & \multicolumn{1}{c|}{--} & 72,616 (13,170)\\[2pt]
% % \hline
% Dev & 4,098 (1,875) & 3,796 (1,255) & 5,658 (1,295)  & 1,784 (492) & 3,718 (778) & 1,874 (478) & \multicolumn{1}{c}{--} \\[2pt]
% % \hline
% Test & 4,101 (2,077) & 7,521 (2,498) & 11,416 (2,595) & 4,107 (1,083) & 7,438 (2,035) & 3,750 (1,414) & \multicolumn{1}{c}{--}\\[2pt]
% % \hline
% Total& 40,989 (16,974) & 11,317 (3,753) & 17,074 (3,890) & 5,891 (1,575) & 11,156 (2,813) & 5,624 (1,892) &  72,616 (13,170)\\[0pt]

\bottomrule
\end{tabular}
% \end{scriptsize}
\end{small}
\caption{Statistics of annotated data. ``\#Pred'' and ``\#Sent'' represent the number of predicates and sentences.} 
\label{data-statistic-anno}
\end{center}
\end{table*}


% \setlength{\tabcolsep}{3.5pt}
% \begin{table}[tb]
% %\setlength{\leftskip}{-25pt}
% \begin{center}
% \begin{small}
% \begin{tabular}{l  c c c c c c }
% \toprule
% & {Source} &{ PB }&{PC}&{ZX}&{LAW}&{MED} \\
% \hline
% Train & 13,022 & -& - & - & - & - \\[2pt]
% % \hline
% Dev & 1,875 & 1,255 & 1,295 & 492 & 778 & 478 \\[2pt]
% % \hline
% Test & 2,077& 2,498 & 2,595 & 1,083 &  2,035& 1,414\\[2pt]
% % \hline
% Total& 16,974 & 3,753 & 3,890 & 1,575 & 2,813 & 1,892 \\[2pt]
% \hline
% % \bottomrule
% \end{tabular}
% \end{small}
% \caption{ Statistics for sentences in COPAD.} 
% \label{data-statistic-target-sentence}
% \end{center}
% \end{table}
